N-1 Security constrained Hosting Capacity Assessment for Ultra Large-scale Data Center with Workload Flexibility

Transmission network security can substantially alter where large-scale data centers can connect and how much workload flexibility can unlock. This paper develops a hosting-capacity framework that couples computing demand, batch workload scheduling, and N-1 security constraints. A modified IEEE 118-bus case study reveals that two data center sites with identical hosting capacities under normal operation differ by 874.5 MW under the contingencies operation when workload flexibility is enabled. Six-hour batch deferral increases N-1 hosting capacity by up to 24.5\% relative to immediate execution. These gains arise from reducing demand at critical hours while accommodating deferred tasks within subsequent transmission limits and deadlines. At bus 92, a four-hour window captures 90.9\% of the six-hour capacity gain. The findings establish workload flexibility as a location-dependent connection resource whose capacity value requires joint assessment of contingency exposure and deadline constrainted workload recovery, beyond the power reduction available at a single critical hour.

==> figures/fig1_batch_security.tex <==
% Conceptual drawing. Rack trays and job symbols are pictograms, not counts.
\begin{tikzpicture}[x=1cm,y=1cm,font=\sffamily\scriptsize,
 wire/.style={line width=.8pt,draw=HCNavy},
 jobpath/.style={draw=HCTeal,densely dashed,line width=.95pt,-{Stealth[length=1.8mm]}},
 pics/rack/.style={code={
   \filldraw[draw=HCNavy,fill=HCNavy!6] (0,0) rectangle (.64,1.04);
   \filldraw[draw=HCNavy,fill=HCNavy!18] (.64,0)--(.85,.13)--(.85,1.17)--(.64,1.04)--cycle;
   \filldraw[draw=HCNavy,fill=white] (0,1.04)--(.21,1.17)--(.85,1.17)--(.64,1.04)--cycle;
   \foreach \y in {.12,.34,.56,.78}{
     \fill[HCNavy!85] (.07,\y) rectangle +(.50,.14);
     \fill[white] (.13,\y+.07) circle (.022);
     \draw[white,line width=.3pt] (.32,\y+.07)--(.50,\y+.07);
   }
 }},
 pics/job/.style={code={
   \filldraw[draw=HCTeal,fill=white] (-.18,-.08) rectangle (.15,.19);
   \filldraw[draw=HCTeal,fill=HCTeal!15] (-.12,-.14) rectangle (.21,.13);
   \draw[HCTeal] (-.06,-.01)--(.14,-.01) (-.06,.055)--(.14,.055);
 }}]
% One enclosure represents a single physical facility across both periods.
\draw[rounded corners=3pt,draw=HCNavy!60,fill=HCNavy!3]
  (2.61,.13) rectangle (9.12,3.93);
\node[anchor=west,font=\sffamily\footnotesize\bfseries,text=HCNavy]
 at (2.79,3.63) {Data center};
\node[anchor=east,text=black!75] at (8.95,3.63) {Same connection site};
\draw[HCNavy!22] (2.83,3.38)--(8.90,3.38);
% Parallel paths between two buses make the outage and supply path explicit.
\draw[HCNavy,line width=1.6pt] (.12,1.13)--(.12,2.49)
 (2.12,1.13)--(2.12,2.49);
\draw[wire,black!50,dashed] (.12,2.34)--(.97,2.34) (1.27,2.34)--(2.12,2.34);
\draw[HCOrange,line width=1.2pt] (.99,2.21)--(1.25,2.47) (.99,2.47)--(1.25,2.21);
\node at (1.12,2.76) {Line outage};
\draw[wire,-{Stealth[length=1.5mm]}] (.12,1.32)--(1.42,1.32);
\draw[wire] (1.42,1.32)--(2.12,1.32);
\node at (1.12,.96) {In-service line};
\draw[wire,-{Stealth[length=1.6mm]}] (2.12,1.81)--(2.82,1.81);
% Ticks align with the arrival and execution symbols below.
\draw[black!65,-{Stealth[length=1.6mm]}] (3.20,2.99)--(8.80,2.99);
\foreach \x in {4.19,7.66}{\draw[black!65] (\x,2.92)--(\x,3.07);}
\node[anchor=east,font=\scriptsize] at (8.72,3.19) {Time};
\pic at (4.19,2.53) {job};
\pic at (7.66,2.53) {job};
\draw[jobpath] (4.49,2.52)--node[midway,fill=HCNavy!3,inner sep=2pt]{Defer batch} (7.34,2.52);
\foreach \x in {3.35,6.82}{
 \pic at (\x+.79,.80) {rack};
 \pic at (\x,.64) {rack};
}
\draw[jobpath] (7.67,2.33)--(7.67,2.01);
\node at (4.18,.35) {Immediate work};
\node at (7.64,.35) {Immediate + batch};
\end{tikzpicture}


==> figures/fig1_framework.tex <==
\begin{tikzpicture}[
    font=\footnotesize,
    >=Latex,
    box/.style={draw, rounded corners=1.5pt, line width=0.6pt,
        align=center, inner xsep=2.0pt, inner ysep=1.5pt},
    input/.style={box, draw=HCNavy, fill=HCLightBlue, text=HCNavy,
        font=\scriptsize,
        minimum height=7.2mm},
    obligation/.style={box, draw=HCOrange, fill=HCLightOrange,
        minimum width=49mm, minimum height=7.2mm},
    scheduler/.style={box, draw=HCOrange, fill=HCLightOrange,
        minimum width=54mm, minimum height=10.0mm},
    physical/.style={box, draw=HCTeal, fill=HCLightTeal,
        minimum width=54mm, minimum height=7.2mm},
    stageone/.style={box, draw=HCNavy, fill=HCLightBlue,
        minimum width=28mm, minimum height=11.0mm},
    stagetwo/.style={box, draw=HCTeal, fill=HCLightTeal,
        minimum width=31mm, minimum height=11.0mm},
    output/.style={box, draw=black!55, fill=HCGray,
        minimum width=59.5mm, minimum height=7.2mm},
    heading/.style={font=\small\bfseries, text=HCNavy},
    flow/.style={->, line width=0.7pt, draw=black!70},
    certify/.style={->, line width=0.8pt, draw=HCOrange}
]

% Capacity-linked service obligation
\node[heading] at (24.5mm,7.2mm) {Capacity-linked service obligation};
\node[input, minimum width=21mm] (capacity) at (10.5mm,0)
    {Admitted DC\\capacity $H_d$};
\node[input, minimum width=27mm] (profile) at (35.5mm,0)
    {Workload intensity\\per MW, $\bar a_{d,t}$};
\node[obligation] (service) at (24.5mm,-10.0mm)
    {Required computational service\\$a_{d,t}=H_d\bar a_{d,t}$};

% Temporal workload-to-power chain
\node[heading] at (82mm,7.2mm) {Temporal workload-to-power chain};
\node[scheduler] (schedule) at (82mm,-1.2mm)
    {\textbf{Service scheduling}\\[-0.2mm]
     Non-Flex: arrival-hour processing\quad$\vert$\quad
     Flex: deadline-constrained deferral $0\leq k\leq K$};
\node[physical] (power) at (82mm,-12.0mm)
    {Processed workload $\rightarrow$ active servers $\rightarrow$
     IT power/PUE $\rightarrow$ nodal DC import};
\node[font=\scriptsize\bfseries, text=HCOrange] at (82mm,-18.0mm)
    {All admitted workloads are completed; no spatial migration};

% Two-stage network assessment
\node[heading] at (143.75mm,7.2mm) {Two-stage network assessment};
\node[stageone] (stage1) at (128mm,-1.7mm)
    {\textbf{Stage 1: HC assessment}\\
     $\displaystyle\max\sum_d H_d$\\[-0.2mm]
     subject to DC-OPF};
\node[stagetwo] (stage2) at (158mm,-1.7mm)
    {\textbf{Stage 2: service schedule}\\
     fix certified $H_d^\star$\\[-0.2mm]
     min. generation + carbon cost};
\node[output] (metrics) at (143.75mm,-14.2mm)
    {HC gain $\vert$ realized deferral $\vert$ critical line-hours};

\draw[flow] (capacity.south) -- ++(0,-2.0mm) -| ([xshift=-9mm]service.north);
\draw[flow] (profile.south) -- ++(0,-2.0mm) -| ([xshift=9mm]service.north);
\draw[flow] (service.east) -- (schedule.west);
\draw[flow] (schedule) -- (power);
\draw[flow] (power.east) -- (stage1.west);
\draw[certify] (stage1.east) -- node[above, font=\scriptsize,
    text=HCOrange] {$H_d^\star$} (stage2.west);
\draw[flow] (stage1.south) |- ([xshift=-12mm]metrics.north);
\draw[flow] (stage2.south) |- ([xshift=12mm]metrics.north);

\end{tikzpicture}

